Verifying Bit-vector Invertibility Conditions in Coq (Extended Abstract)

This work is a part of an ongoing effort to prove the correctness of invertibility conditions for the theory of fixed-width bit-vectors, which are used to solve quantified bit-vector formulas in the Satisfiability Modulo Theories (SMT) solver CVC4. While many of these were proved in a completely automatic fashion for any bit-width, some were only proved for bit-widths up to 65, even though they are being used to solve formulas over arbitrary bit-widths. In this paper we describe our initial efforts in proving a subset of these invertibility conditions in the Coq proof assistant. We describe the Coq library that we use, as well as the extensions that we introduced to it.

==> eptcsdata.tex <==
\providecommand{\firstpage}{18}
\providecommand{\publicationstatus}{Haniel Barbosa and Giselle Reis (Eds.): Sixth Workshop\\ on Proof eXchange for Theorem Proving (PxTP)\\
EPTCS 301, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.301.4}{10.4204/EPTCS.301.4}}
\pdfoutput=1

